UniTE -- The Best of Both Worlds: Unifying Function-Fitting and Aggregation-Based Approaches to Travel Time and Travel Speed Estimation

Travel time or speed estimation are part of many intelligent transportation applications. Existing estimation approaches rely on either function fitting or aggregation and represent different trade-offs between generalizability and accuracy. Function-fitting approaches learn functions that map feature vectors of, e.g., routes, to travel time or speed estimates, which enables generalization to unseen routes. However, mapping functions are imperfect and offer poor accuracy in practice. Aggregation-based approaches instead form estimates by aggregating historical data, e.g., traversal data for routes. This enables very high accuracy given sufficient data. However, they rely on simplistic heuristics when insufficient data is available, yielding poor generalizability. We present a Unifying approach to Travel time and speed Estimation (UniTE) that combines function-fitting and aggregation-based approaches into a unified framework that aims to achieve the generalizability of function-fitting approaches and the accuracy of aggregation-based approaches. An empirical study finds that an instance of UniTE can improve the accuracies of travel speed distribution and travel time estimation by $40-64\%$ and $3-23\%$, respectively, compared to using function fitting or aggregation alone

==> acknowledgments.tex <==
%\begin{acks}
\section{Acknowledgments}
  The research presented in this paper is supported in part by the DiCyPS project and by grants from the Obel Family Foundation and VILLUM FONDEN.
We also thank the \glsfirst{osm} contributors who have made this work possible.
%Map data is copyrighted by the OpenStreetMap contributors and is available from {https://www.openstreetmap.org}.
%\end{acks}


==> discussion.tex <==
\section{Discussion}
\begin{itemize}
    \todo{Mention in method and possibly under experiments. Point in AGHA section that this is apparent from, e.g., the computation of the mean.}
    \item We have not tested with state-of-the-art methods
    \item Doesn't matter, our approach is theoretically guaranteed to be no worse than either approach.
    \item Function-fitting: Express extremely high confidence in the prior
    \item Aggregation-based: Express extremely low confidence in the prior
\end{itemize}


==> gaussian_mixture_derivation.tex <==
\section{Hybrid Driving Speed Estimation}
Model-based approaches aim to learn the model parameters $\theta$ that best explain the relationship between the unknown future driving speed $d_i$ when traversing route $p_i$ and the feature vector representation $\mathbf{p}_i$ of route $p_i$.
Formally, the model parameters $\theta$ are chosen to maximize the conditional likelihood
\begin{equation}\label{eq:model-based}
  \prod_{i=1}^n \Pr(d_i \mid \mathbf{p}_i; \theta)
\end{equation}
based on a set of $n$ training trajectories.
The probability density $\Pr(d_i \mid \mathbf{p}_i; \theta)$ may for instance be computed using forward propagation through a neural network with input $\mathbf{p}_i$ and network weights $\theta$.
By sharing model parameters across training trajectories during optimization, model-based approaches can generalize to any unseen routes.

Aggregation-based approaches aim to learn model parameters $\theta_i$ for each route in the set of training trajectories.
In other words, given a set of $n$ training trajectories, instance-based approaches solve $n$ optimization problems.
For the $i$th training trajectory, $\theta_i$ is chosen s.t.\ it is the maximum a posteriori probability (MAP) estimate of
\begin{equation}\label{eq:aggregation-based}
  \Pr(\theta_i \mid \tilde{D}_i)
\end{equation}
where $\tilde{D}_i$ is a set of historical driving speeds.
The driving speeds in $\tilde{D}_i$ are typically collected from other trajectories traversing route $p_i$.
By using distinct model parameters for each route in the set of training trajectories, aggregation-based approaches can learn a more accurate representation of the driving speed distribution of $d_i$ provided they have enough data.
Unfortunately, aggregation-based approaches rely on simple heuristics to provide reasonable estimates for unseen routes and are prone to overfit when only a few historical driving speeds are available.

In this work, we present a hybrid approach that leverages the generalizability of model-based driving speed estimation with the accuracy of aggregation-based approaches.
Given a set of $n$ training trajectories, we aim to learn model parameters $\theta$ s.t.\ $\theta$ maximizes the conditional likelihood
\begin{equation}
  \prod_{i=1}^n \Pr(d_i \mid \tilde{D}_i)
\end{equation}
where 
\begin{equation}
  \begin{split}
    \prod_{i=1}^n \Pr(d_i \mid \tilde{D}_i) &= \prod_{i=1}^n \int\Pr(d_i \mid \theta_i, \tilde{D}_i) \Pr(\theta_i \mid \tilde{D}_i; f(\mathbf{p}_i, \theta)) \mathit{d\theta_i} \\
                              &= \prod_{i=1}^n \int\Pr(d_i \mid \theta_i, \tilde{D}_i) \frac{\Pr(\theta_i; f(\mathbf{p}_i, \theta)) \Pr(D \mid \theta_i)}{\Pr(D)} \mathit{d\theta_i}
  \end{split}
\end{equation}
In essence, we parameterize the computation of the 
Compared to \cref{eq:}
In essence, we have parameterized the di
Here, $\Theta$ is a function of the 

\section{Problem Formulation}
In this work, we aim to combine the model-based approach and instance-based approach into a hybrid approach to predict time-varying driving speeds when traversing edges and routes.

Model-based approach typically learn a discriminative model of the form
\begin{equation}
  \Pr(d \mid \mathbf{p}, \theta)
\end{equation}
where $d$ is the driving speed when traversing route $p$ (i.e., a path or an edge) at time $\tau$, and $\theta$ are the model parameters, e.g., the weights in a neural network.
The vector $\mathbf{p}$ is a time-varying $d$-dimensional feature vector of route $p$.

The model parameters $\theta$ may be learned using maximum likelihood estimation by finding the parameters $\theta$ that maximizes the likelihood
\begin{equation}
  \Pr(D \mid \theta) = \prod_{i=1}^n \Pr(d_i \mid \mathbf{p}_i, \theta)
\end{equation}
where $d_i$ is driving speed when traversing route $p_i$.
The driving speeds $D = \{d_1, \dots, d_n\}$ are assumed to be independent and identically distributed. 

In this work, we aim to condition the likelihood not only on the model parameters $\theta$ but also on set of relevant instances $\tilde{\mathcal{D}}=\{\tilde{D}_1, \dots, \tilde{D}_n \}$.
Formally, we use maximum likelihood estimation to find the parameters $\theta$ that maximizes the likelihood
\begin{equation}\label{eq:prob-form-hybrid}
  \Pr(D \mid \theta, \tilde{\mathcal{D}}) = \prod_{i=1}^n \Pr(d_i \mid \mathbf{p}_i, \theta, \tilde{D}_i)
\end{equation}
where $\tilde{D}_i \subseteq D \setminus \{d_i\} $ is a (possibly empty) set of driving speed samples that are relevant to the prediction of driving speed $d_i$ and serve as extra input data.
\todo{The evidence being subset of the data is unusual and should probably be commented on.}
For instance, $\tilde{D}_i$ may be driving speed samples from route $p_i$ within a time interval around time $\tau$.
We discuss possible ways to select $\tilde{D}_i$ in \cref{sec:data-selection}.

\todo{Maybe mixture density networks are related and could help the reader.}

\subsection{Gaussian Mixture with Component Normal-Gamma Priors}
In this work, we assume that the distribution of driving speeds follows a $K$-component Gaussian mixture model, i.e., that
%\begin{equation}
\begin{equation}
  \Pr(d \mid \mathbf{p}, \theta, \tilde{D}) = \\
    \sum_{k=1}^K w_{m, k} \Pr(d \mid Z=k, \mathbf{p}, \theta, \tilde{D}) 
\end{equation}
%\end{equation}
where $w_{m, k} = \Pr(Z=k \mid \mathbf{p}, \theta, \tilde{D})$ is the weight of the $k$th component after observing relevant driving samples
$\tilde{D} = \{\tilde{d}_1, \dots, \tilde{d}_m\}$.
A component in the mixture can represent, e.g., samples where the driver that had to stop at an intersection, and another component may represent those who could travel through the intersection uninhibited.

We assume that this probability distribution of driving speed $d_i$ follows 


\begin{figure*}
  \centering
  \input{illustrations/conceptual_framework.tikz.tex}
  \caption{\label{fig:conceptual-framework}}
\end{figure*}


Let $E = \{ d_1, \dots, d_n \}$ be the evidence to be inserted.
Let $\boldsymbol\mu = [\mu_1 \dots \mu_K]$ and $\boldsymbol{\lambda} = [\lambda_1 \dots \lambda_K]$ denote component means and component precisions, respectively, of a $K$-component Gaussian mixture.
Let $\mathbf{w} = [w_1 \dots w_K]$ denote component weights s.t.\ $w_k = \Pr(C_k)$ is the prior probability of the $k$th component.

We want to compute the posterior predictive distribution of a Gaussian mixture.
\begin{equation}
  \begin{split}
    \Pr(d \mid E=\{d_1, \dots, d_n\}) = \sum_{k=1}^K \Pr(C_k \mid E) \Pr(d \mid C_k, E) \\
  \end{split}
\end{equation}
where $\Pr(d \mid C_k, E)$ is the posterior predictive distribution of the $k$th Gaussian component in the distribution.
Note, that in the case of a single-component Gaussian, $\Pr(d \mid C_k, E) = \Pr(d \mid E)$ which is a student's $t$-distribution as described in \cref{sec:parameter-estimation-gaussian}.
\cref{sec:parameter-estimation-gaussian} describes how to compute the posterior predictive of a Gaussian from which all the samples in $E$ originates.
Updating all the components based on $E$ results in a convergence to a single Gaussian, thus losing expressibility of the mixture.
The challenge is therefore to partition $E$ into $K$ partitions, one for each component, s.t.\ the $k$th component can be updated based on the $k$th.

Partitioning $E$ is non-trivial since there is uncertainty as to which component a sample $d_i \in E$ originates from.
Thankfully, this problem has been studied in the context of fitting Gaussian Mixture Models using an Expectation-Maximization approach~\citep{murphy-mixtures}.
Here, each component $C_k$ is given a \emph{responsibility score} $r_{k,i}$ for each sample $d_i$ s.t.\
\begin{equation}
  \begin{split}
    r_{k, i} &= \Pr(C_k \mid d_i) \\
             &= \frac{\Pr(d_i, C_k)}{\Pr(d_i)} \\
             &= \frac{\Pr(d_i \mid C_k)\Pr(C_k)}{\sum_{l=1}^K \Pr(d_i \mid C_l)\Pr(C_l)}.
  \end{split}
\end{equation}
In other words, the responsibility score $r_{k, i}$ is the probability that driving speed sample $d_i \in E$ originates from component $C_k$.

When updating a component using the rules in \cref{eq:parameter-update}, we use the responsibility scores to compute
\emph{responsible sample size} $n_k = \sum_{i=1}^n r_{k, i}$,
\emph{responsible sample mean} $\mu_{E, k} = \frac{\sum_{i=1}^n r_{k, i}d_i}{n_k}$, and
\emph{responsible sample variance} $\sigma^2_{E, k} = \frac{\sum_{i=1}^n r_{k, i} {(d_i - \mu_{E, k})}^2}{n_k}$
to replace the sample size $n$, sample mean $\mu_E$, and sample variance $\sigma^2_E$, respectively.
From this perspective, each driving speed sample $d_i \in E$ is soft-assigned to a component where the confidence in the assignment is given by $r_{k,i}$.
Effectively, each component is therefore updated on different partitions of the data and thereby avoids component convergence towards the sample single Gaussian.
In addition, substituting $n_k$, $\mu_{E, k}$, and $\sigma^2_{E, k}$ for $n$, $\mu_{E}$ and $\sigma^2_E$, respectively, has no effect in the single component case.

In summary, we compute the posterior predictive of a Gaussian mixture, i.e.,
\begin{equation}
  \begin{split}
    \Pr(d \mid E=\{d_1, \dots, d_n\}) &= \sum_{k=1}^K \Pr(C_k \mid E) \Pr(d \mid C_k, E) \\
                                      &= \sum_{k=1}^K w_{n, k} T_{2\alpha_{n, k}}(d \mid \mu_{n, k}, \frac{\beta_{n, k}(\kappa_{n, k} + 1)}{\alpha_{n, k}\kappa_{n, k}})
  \end{split}
\end{equation}
where 
\begin{equation}
\begin{split}
  w_{n, k} &= \Pr(C_k \mid E) \\
           &= \frac{\Pr(E \mid C_k)\Pr(C_k)}
                   {\Pr(E)} \\
           &= \frac{\Pr(C_k)  \prod_{i=1}^n \Pr(d_i \mid C_k)}
                   {\prod_{i=1}^n  \sum_{l=1}^K \Pr(d_i \mid C_l) \Pr(C_l)} \\
           &= \frac{w_{0, k}  \prod_{i=1}^n T_{2\alpha_{0, k}}(d_i \mid \mu_{0, k}, \frac{\beta_{0, k}(\kappa_{0, k} + 1)}{\alpha_{0, k}\kappa_{0, k}})}
                   {\prod_{i=1}^n  \sum_{l=1}^K T_{2\alpha_{0, k}}(d_i \mid \mu_{0, l}, \frac{\beta_{0, l}(\kappa_{0, l} + 1)}{\alpha_{0, l}\kappa_{0, l}}) w_{0, l}} \\
  \mu_{n, k}    &= \frac{\kappa_{0,k} \mu_{0,k} + n_k \mu_{E, k}}
                        {\kappa_{0,k} + n_k} \\
  \kappa_{n, k} &= \kappa_{0,k} + n_k \\
  \alpha_{n, k} &= \alpha_{0,k} + \frac{n_k}{2} \\
  \beta_{n, k} &= \beta_{0,k} +
             \frac{1}{2} n_k \sigma^2_{E,k} +
             \frac{1}{2}\frac{\kappa_{0,k} n_k {(\mu_{E, k} - \mu_{0, k})}^2}
                             {\kappa_{0,k} + n_k}
\end{split}
\end{equation}

\COMMENT{
First, we consider the single-component case and model the evidence $E = \{d_1, \dots, d_n \}$ as a random variable where the probability of sampling a driving speed $d_i \in E$ is uniform, i.e., $\Pr(E=d_i) = \frac{1}{n}$.
In this case, we can rewrite the rules for posterior parameters s.t.\ they are expressed in terms of random variable $E$, i.e.,
\begin{equation}\label{eq:reformulated-parameter-update}
\begin{split}
  \mu_n    =& \frac{\kappa_0 \mu_0 + n \mu_E}
                   {\kappa_0 + n} \\
  \kappa_n =& \kappa_0 + n \\
  \alpha_n =& \alpha_0 + \frac{n}{2}\\
  \beta_n =& \beta_0 +
             \frac{1}{2}n_E\sigma^2_E +
             \frac{1}{2}\frac{\kappa_0 n {(\mu_E - \mu_0)}^2}
                             {\kappa_0 + n}
\end{split}
\end{equation}
where $E = \{d_1, \dots, d_n\}$ is the driving speed samples given as evidence,
%$n_E = \sum_{i=1}^n \Pr(E=d_i) n$ is the number of samples,
$\mu_E = \mathbb{E}[E] = \sum_{i=1}{n} \Pr(E=d_i) d_i$ is the sample mean, and $\sigma^2_E = Var(E) = \sum_{i=1}^n \Pr(E=d_i){(d_i - \mu_E)}^2$ is the biased sample variance.

Next, we extend the rules in \cref{eq:reformulated-parameter-update} to the multi-component case.
To update a Gaussian component $C_k$ in this case, we must model the uncertainty of the evidence, represented by random variable $E$, originates from $C_k$.
To do this, we replace random variable $E$ in \cref{eq:reformulated-parameter-update} with conditional random variable $E \mid C_k$ with probability distribution
\begin{equation}
    \Pr(E=d_i \mid C_k) = \frac{\Pr(C_k \mid D=d_i)}{\sum_{j=1}^n \Pr(C_k \mid D=d_j)} 
\end{equation}
where 
\begin{equation*}
  \begin{split}
    \Pr(C_k \mid D=d_i) &= \frac{\Pr(D=d_i, C_k)}{\Pr(D=d_i)} \\
                        &= \frac{\Pr(D=d_i \mid C_k)\Pr(C_k)}{\sum_{l=1}^K \Pr(D=d_i \mid C_k)}
  \end{split}
\end{equation*}
The probability $\Pr(E=d_i \mid C_k)$ denotes the probability of sampling driving speed sample $d_i \in E$ from random variable $E$ given that the samples are generated by component $C_k$.
In other words, the probability of samples $d_i \in E$ is no longer uniform, but proportional to their probability density w.r.t.\ the component being updated.
In summary, the posterior parameters of the $k$th Gaussian component of the mixture is
\begin{equation}\label{eq:component-parameter-update}
\begin{split}
  \mu_{n, k}    =& \frac{\kappa_{0,k} \mu_{0,k} + n \mu_{E \mid C_k}}
                        {\kappa_{0,k} + n} \\
  \kappa_{n, k} =& \kappa_{0,k} + n \\
  \alpha_{n, k} =& \alpha_{0,k} + \frac{n}{2} \\
  \beta_{n, k} =& \beta_{0,k} +
             \frac{1}{2} n_E \sigma^2_{E \mid C_k} +
             \frac{1}{2}\frac{\kappa_{0,k} n {(\mu_{E \mid C_k} - \mu_{0, k})}^2}
                             {\kappa_{0,k} + n}
\end{split}
\end{equation}
where
\begin{equation*}
  \begin{split}
    %n_{E \mid C_k} &= \sum_{i=1}^n \Pr(E=d_i \mid C_k) n, \\
    \mu_{E \mid C_k} &= \sum_{i=1}^n{\Pr(E=d_i \mid C_k) d_i}\text{, and} \\
    \sigma^2_{E \mid C_k} &= \sum_{i=1}^n{\Pr(E=d_i \mid C_k)} {(d_i - \mu_{E \mid C_k})}^2.
  \end{split}
\end{equation*}
}

\section{Interesting Properties}
Interesting regularization: Model will have little influence on loss in cases where there is a lot of data, encouraging better performance in areas with little data.
These areas are precisely where a model-based approach is required.


==> illustrations/model_based_architecture.tikz.tex <==
\usetikzlibrary{bayesnet,arrows,positioning,shapes}
\begin{tikzpicture}[thick]
\end{tikzpicture}


==> notes.tex <==
\section{Notes}

\subsection{Observations}
\begin{enumerate}
  \item Driving speeds of adjacent segments tend to be correlated, but not necessarily similar
  \item In a vehicle trajectory, the driving speed when traversing a road segment is influenced by how the vehicle arrives and departs from the segment. This includes, e.g., acceleration due to a difference in speed limits or traffic conditions, the angle of a turn, or the presence of a traffic light at the connecting segments.
  \item Vehicle trajectories are often incomplete such that short road segments are more likely to travel time information than long road segments.
  \item Only a few paths will have sufficient trajectory data to adequately estimate the travel time distribution of a path. Even individual edges are likely to lack sufficient trajectory data. However, given enough data, the data may provide a very rich source of information that captures non-obvious information of an edge or path. For instance, the type of drivers that generally drive there. 
  \item Travel time when traversing a road segment is highly time-dependent.
\end{enumerate}

\subsection{Proposal 1: Observation Update a Prior Estimated by a Neural Network}
Estimates a $k$-component Gaussian Mixture for each road segment in a route. Each mixture can subsequently be updated based on any relevant trajectory data, e.g., all historical trajectories that have taken the route. Finally, the travel time distribution of the route is computed by summing over the mixtures of each road segment in the route (this step is very expensive, $k^{|R|}$, where $|R|$ is the length of the route. Possible Monte Carlo approximation, but maybe not so satisfying. Also not clear how to make a joint per-segment travel time loss and per-trajectory loss).

This idea is computationally feasible with point estimates, but requires assuming segment driving speeds are Gaussian (which they often are not).


% Links:
%% https://stats.stackexchange.com/questions/174791/sum-of-gaussian-mixture-and-gaussian-scale-mixture
%% https://publications.aston.ac.uk/id/eprint/373/1/NCRG_94_004.pdf

\subsection{Proposal 2: Treat Observations as a Particular Attribute}



==> observational_update.tex <==
\section{Hybrid Travel Time Estimation}
We model the driving speed $D$ of a road segment $e$ as a random variable variable with probability distribution $\Pr(D \mid \theta)$ where $\theta$ is the set of distribution parameters.
Our framework estimates $\theta$ using a model $f$ and adjusts this estimate based on a set driving speed samples $\{d_1, \dots, d_n\}$ from $D$.

\begin{figure}[h]
  \centering
  \input{illustrations/conceptual_framework.tikz.tex}
  \caption{Overview of our method in plate notation.\label{fig:update-overview}}
\end{figure}

\cref{fig:update-overview} illustrates our framework using plate notation.
In the figure, a model $f$ takes as input an edge $e$ and generates set of prior parameters $\theta_0$ without considering any driving speed samples.
These prior parameters parameterize the prior probability $\Pr(D \mid \theta_0)$.
In practice, the model $f$ is unlikely to be perfect.
Therefore, any available driving speed samples $E=\{d_1, \dots, d_n\}$ are inserted as evidence, as illustrated in \cref{fig:update-overview}.
The resulting posterior probability $\Pr(D \mid E, \theta_0) = \Pr(D \mid \theta_n)$ is used as the hybrid model output.
We refer to $\theta_n$ as posterior parameters.

The framework we propose is hybrid in the sense that it can use a model $f$ to predict prior parameters for the distribution of the driving speed $D$, but it can also use driving speed samples observed during training to adjust these parameters.
We have only talked of the model $f$ of being dependent on the road segment $e$.
In practice $f$ may also depend on other factors, such as the time of day or the information about the driver.

\subsection{Estimating Driving Speed Distributions}
We model a driving speed distribution $\Pr(D \mid \theta)$ as a uni-variate Gaussian mixture with $K$ components.
In a Gaussian mixture, the probability of a driving speed $d$ is a weighted mean of the probability of $d$ originating from each component, i.e.,
\begin{equation*}
  \Pr(D=d \mid \theta) = \sum_{k=1}^K w_k \Pr(D=d \mid \theta_k)
\end{equation*}
where $\sum_{k=1}^K w_k = 1$ and $\theta_k \in \theta$ is the set of parameters for the $k$th component.
In practice, the mean and variance of the driving speed is unknown, since driving speed data is incomplete and may also be noisy.
Consequently, the mean and variance of each Gaussian component is also unknown.

\subsubsection{Bayesian Parameter Estimation of a Gaussian}\label{sec:parameter-estimation-gaussian}
% Based on: https://www.cs.ubc.ca/~murphyk/Papers/bayesGauss.pdf
We first consider the case of estimating the parameters of a single-component mixture, i.e., a single uni-variate Gaussian distribution with unknown mean and variance.
For this case, there exists a well-known approach based on Bayesian inference in conjunction with conjugate priors, i.e., priors of the form $\Pr(\theta)$ that belong to the same distribution family as their posterior $\Pr(\theta \mid E)$.
The use of conjugate priors allows closed-form derivation of the posterior distribution parameters which can be computed efficiently and are differentiable.
Differentiability is desirable since makes it possible to train the model $f$ to be jointly with the estimation of the posterior parameters.

Let $\Pr(D \mid \mu, \lambda)$ denote a Gaussian driving speed distribution with mean $\mu$ and variance $\sigma^2$.
We use the following normal-gamma prior to estimate $\mu$ and $\lambda$.
\begin{equation}\label{eq:conjugate-priors}
  \mathit{NG}(\mu, \lambda \mid \mu_0, \kappa_0, \alpha_0, \beta_0) =
  \mathcal{N}(\mu \mid \mu_0, \frac{1}{\kappa_0\lambda_0})
  \mathit{Ga}(\lambda \mid \alpha_0, \beta_0).
\end{equation}
Note, that, for ease of notation, we use the precision $\lambda = \frac{1}{\sigma^2}$, shape parameter $\alpha_0$, rate parameter $\beta_0$ to parameterize the normal-gamma prior distribution.
Also note that \cref{eq:conjugate-priors} is only defined for $\kappa_0 > 0$, $\alpha_0 > 0$, and $\beta_0 > 0$.

In \cref{eq:conjugate-priors}, model $f$ is required to output the prior parameters $\mu_0$, $\kappa_0$, $\alpha_0$, and $\beta_0$.
The prior parameters represent prior beliefs about the mean $\mu$ and precision $\lambda$ of a Gaussian distribution. After observing driving speed samples $E = \{d_1, \dots, d_n\}$ (for $n \geq 0 $), confidence in the values of $\mu$ and $\lambda$ will change. Formally, the prior parameters are updated as follows.
\begin{equation}\label{eq:parameter-update}
\begin{split}
  \mu_n    =& \frac{\kappa_0\mu_0 + n\bar{d}}
                   {\kappa_0 + n} \\
  \kappa_n =& \kappa_0 + n \\
  \alpha_n =& \alpha_0 + \frac{n}{2}\\
  \beta_n =& \beta_0 +
             \frac{1}{2}nS^2 +
             \frac{1}{2}\frac{\kappa_0n{(\bar{d} - \mu_0)}^2}
                             {\kappa_0 + n}
\end{split}
\end{equation}
where $\bar{d} = \frac{\sum_{i=2}^n d_i}{n}$ is the sample mean and $S^2 = \frac{\sum_i^n{(d_i - \bar{d})}^2}{n}$ is the biased sample variance.
Note that if there is no data, i.e., $n = 0$, then none of the prior parameters are updated in \cref{eq:parameter-update}.

After observing driving speed samples $E = (d_1, \dots, d_n)$, the driving speed $D$ follows a student's $t$-distribution, s.t., the probability of driving speed $d$ is
\begin{equation}
\begin{split}
  \Pr(D=d \mid \mu_n, \kappa_n, \alpha_n, \beta_n) & = t_{\nu}(d \mid \hat{\mu}, \hat{\sigma}) \\
    & =
    \frac{\Gamma(\frac{\nu +1}{2})}
         {\Gamma(\frac{\nu}{2}) \sqrt{\nu \pi} \hat{\sigma} }  % times
    {\Bigg(
        1 + \frac{1}{\nu}  % times
        {\Big( \frac{d - \hat{\mu}}{\hat{\sigma}} \Big)}^2 
    \Bigg)}^{-\frac{\nu+1}{2}}.
\end{split}
\end{equation}
where $\Gamma$ is the gamma function and $\nu$, $\hat{\mu}$, and $\hat{\sigma}$ are, respectively, the degrees of freedom, the center, and the scale of the distribution.

\subsubsection{Bayesian Parameter Estimation of a Gaussian Mixture}
It is well-established in the literature that driving speeds do not follow any simple distribution, such as a Gaussian.
We therefore extend the single-component approach described in \cref{sec:parameter-estimation-gaussian} to the Gaussian mixture case.
In this case, the model $f$ is required to output prior parameters $w_{0, k}, k$, $\mu_{0, k}$, $\lambda_{0, k}$, $\alpha_{0, k}$, and $\beta_{0, k}$ for each component $C_k$ in the $K$-component mixture s.t.\ the probability density function of the mixture is 
\begin{equation}
    \Pr(D=d \mid \theta_0) = \sum_{k=1}^K \Pr(C_k \mid w_{0, k}) \Pr(D=d \mid \mu_{0, k}, \lambda_{0, k}, \alpha_{0, k}, \beta_{0, k})
\end{equation}
where $\Pr(C_k \mid w_{0, k}) = w_{0, k}$.

After observing $n$ driving speed observations $E = \{d_1, \dots, d_n\}$ as evidence, we are interested in the posterior distribution
\begin{equation}
  \begin{split}
    \Pr(D=d \mid E, \theta_0) &= \Pr(D=d \mid \theta_n) \\ 
    %\sum_{k=1}^K \Pr(C_k \mid E, w_{0, k}) \Pr(D=d \mid E, \mu_{0, k}, \lambda_{0, k}, \alpha_{0, k}, \beta_{0, k}) \\ 
                              &= \sum_{k=1}^K \Pr(C_k \mid w_{n, k}) \Pr(D=d \mid\mu_{n, k}, \lambda_{n, k}, \alpha_{n, k}, \beta_{n, k})
  \end{split}
\end{equation}
where the posterior parameters are $w_{n, k}$, $\mu_{n, k}$, $\lambda_{n, k}$, $\alpha_{n, k}$, and $\beta_{n, k}$.

In brief, we introduce an update rule for the component weight of a Gaussian component $C_k$ in the mixture.
In addition, we modify the update rules in \cref{eq:parameter-update} s.t.\ the effect of a driving speed sample $d$ on the update of the prior parameters of a component $C_k$ is proportional to the probability $\Pr(C_k \mid d)$ that $d$ is generated by that component.
This ensures that the component means and variances do not all converge towards the sample mean and sample variance when there are is more than one component.

Given evidence $E = \{d_1, \dots, d_n\}$, we compute the posterior parameters of each Gaussian component $C_k$ in the mixture as follows.
\begin{equation}\label{eq:mixture-component-update}
\begin{split}
  w_n &= \frac{\kappa_0 w_0 + nw_d}
                   {\kappa_0 + n} \\
  \mu_n    &= \frac{\kappa_0 \mu_0 + n\bar{d}}
                   {\kappa_0 + n} \\
  \kappa_n &= \kappa_0 + n \\
  \alpha_n &= \alpha_0 + \frac{n}{2} \\
  \beta_n &= \beta_0 +
             \frac{1}{2} n S^2 +
             \frac{1}{2}\frac{\kappa_0 n {(\bar{d} - \mu_0)}^2}
                             {\kappa_0 + n}
\end{split}
\end{equation}
where
\begin{equation*}
  \begin{split}
    nw_d &= \Pr(C_k) = \sum_{i=1}^n\frac{\Pr(C_k \mid d_i)}{\sum_{j=1}^K\Pr(C_j \mid d_i)} \\
    %p &= \sum_{i=1}^n \frac{{\Pr(C_k \mid d_i)}}
    %                       {\sum_{j=1}^K \Pr(C_j \mid d_i)}, \\
    \bar{d} &= \frac{\sum_{i=1}^n \Pr(C_k \mid d_i) x_i}{\sum_{j=1}^n \Pr(C_k \mid d_j)}, \text{and} \\
    S^2 &= \frac{\sum_{i=1}^n{\Pr(C_k \mid d_i)(d_i - \bar{d})}^2}{\sum_{j=1}^n \Pr(C_k \mid d_j)}.
  \end{split}
\end{equation*}
Here, $w_d$ represents the component weight of component $C_k$ when estimated from the evidence $E$, and $p$ is a pseudo count representing the expected number of driving speed samples to have originated from component $C_k$.
Similarly, $\bar{d}_k$ and $S^2_k$ is the expected sample mean and expected biased sample variance of the samples originating from component $C_k$.

The primary differences between the Gaussian update rules in \cref{eq:parameter-update} and the Gaussian component update rules in \cref{eq:mixture-component-update} is that
\begin{enumerate}
  \item an update rule for the component weights in the mixture is introduced, and
  \item that the influence of the given samples in the update of a component $C_k$ is proportional to the number of expected samples originating from $C_k$.
\end{enumerate}
In other words, the samples given as evidence do not increase certainty about the mean $\mu$ and the variance $\sigma^2$ of component $C_k$ substantially if the samples are unlikely to have originated from $C_k$.

\subsubsection{Joint Model Training}
TODO
\begin{itemize}
  \item Prior and posterior loss
  \item Initialization
  \item Shared $kappa_0$
  \item Regularization
\end{itemize}


\subsubsection{Sample Selection}
TODO



==> pvldb/license.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%


==> record_selection.tex <==
\section{Record Selection Algorithm}\label{app:record-selection-algorithm}
The AGG algorithm and the \gls{aha} variants used in our empirical study (see \cref{sec:exp-algos}) rely on a record selection strategy to find historical records to compute posterior hyperparameters.
The algorithm used for record selection is presented in \cref{alg:record-selection}.

The record selection algorithm takes as input training trajectories $\mathcal{T}$, the route $p$ for which travel time is in the process of being estimated, the road segment $e_i \in p$ for which historical records $\tilde{T}_i$ are currently being selected, and the arrival time $\tau_i$ at road segment $e_i$.
In addition, the algorithm takes as input two parameters: an integer contextual relevance parameter, $c$, and a temporal relevance parameter, $\delta$, in some unit of time.

Recall, from \cref{sec:exp-algos} that the contextual and temporal relevance hyperparameters $c$ and $\delta$ adjust the record selection strategy's emphasis on record relevance and record availability.
For instance, higher values of $\delta$ typically result in more historical records being selected, but they are less indicative of the ground truth travel speed distribution.
Similarly, lower values of $c$ also typically result in more historical records being selected, but they are less contextually relevant where context refers to the preceding and succeeding road segments in the trajectory from which the historical record originated.

\begin{algorithm}
  \caption{Record Selection\label{alg:record-selection}}
  \begin{algorithmic}[1]\raggedright
    \Function{RecordSelection}{$\mathcal{T}$, $p=(e_1, \dots, e_q)$; $e_i$, $\tau_i$ $c$, $\delta$}
        \State{$\tilde{T}_i \gets \emptyset$}
        \State{$C_i \gets (e_{i-c}, \dots, e_{i-1}, e_i, e_{i+1}, \dots, e_{i+c})$}\label{line:record-selection-context-i}
        \ForEach{trajectory $T \in \mathcal{T}$}
            \State{\Let{$T = \big((e'_1, \tau_1, t_1), \dots, (e'_n, \tau_n, t_n)\big)$}}
            \For{$j = 1$ to $n$}
                \State{$C_j \gets (e'_{j-c}, \dots, e'_{j-1}, e'_j, e'_{j+1}, \dots, e'_{j+c})$}
                \If{$C_i = C_j$}
                    \If{$\tau_i - \frac{\delta}{2} \leq \tau_j \leq \tau_i + \frac{\delta}{2}$}
                        \If{$t_i \neq \varnothing$}
                            \State{$\tilde{T}_i \gets \tilde{T}_i \cup \{t_i  \}$}
                        \EndIf
                   \EndIf
                \EndIf
            \EndFor
        \EndFor
        \State{\Return{$\tilde{T}_i$}}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

Given the necessary inputs, the record selection algorithm in \cref{alg:record-selection} proceeds to construct the set of historical records $\tilde{T}_i$ as follows.
First, it stores the context of road segment $e_i$ in variable $C_i$ on Line~$3$.
Then, the algorithm scans the set of training trajectories in the loop on {Lines~$4$-$11$} for historical records.
For each trajectory, the algorithm scans each traversal in the trajectory for historical records in the loop on {Lines~$6$-$11$}.
A historical record refers strictly to the recorded travel time or travel speed of the traversal.

To be selected, a historical record must satisfy two conditions.
First, it must be \emph{contextually relevant}, i.e.,from a traversal of road segment $e_i$ and have the same $c$ preceding and succeeding road segments in trajectory $T$ as $e_i$ in route $p$.
This check is performed by comparing the contexts of the traversal $C_j$ with that of the road segment $C_i$ on {Lines~7-8} of \cref{alg:record-selection}.
Second, the historical record must be \emph{temporally relevant}, i.e., occur at a similar time of week as $\tau_i$
This check is performed on Line~9.
Finally, the historical record is added to $\tilde{T}_i$ on Line~$11$ if $t_i \neq \varnothing$, i.e., that the historical record is derived from \gls{gps} data rather than the map-matching algorithm.
During training, $t_i$ is excluded from $\tilde{T}_i$ if it originates from the trajectory currently being forward propagated.


==> representation_of_time.tex <==
\section{Time of Week Vector Representation}\label{app:representation-of-time}
As explained in \cref{sec:representation-of-time}, we learn a $16$-dimensional time of week vector representation, where $8$ dimensions are used to represent the time of day and $8$ dimensions are used to represent the time of the week.

Formally, we learn a time-of-week vector
\begin{equation}
 \boldsymbol\tau_{\mathit{tow}} = \boldsymbol\tau_{\mathit{tod}} \oplus \boldsymbol\tau_{\mathit{dow}}
\end{equation}
for time $\tau$, where $\boldsymbol\tau_{\mathit{tod}} \in \mathbb{R}^8$ represents the time of day, $\boldsymbol\tau_{\mathit{dow}} \in \mathbb{R}^8$ represents the day of the week, and $\oplus$ denotes vector concatenation.

\subsection{Time of Day Representation}
To represent time of day in our experiments, we divide the time of day into $96$ $15$-minute intervals $\mathcal{I} = \{I_1, \dots, I_{96} \}$ s.t.\ interval $I_1 = \interval{0:00}{0:15}$, $I_2 = \interval{0:15}{0:30}$, and so forth.
Then, we one-hot encode the time of day $\tau_{\mathit{tod}}$ into a $96$-dimensional vector $\boldsymbol\tau'_{tod} = \begin{bmatrix} \mathbbm{1}[\tau_{\mathit{tod}} \in I_1] & \dots & \mathbbm{1}[\tau_{\mathit{tod}} \in I_{96}] \end{bmatrix}$ where $\mathbbm{1}$ is the indicator function.
Finally, we multiply the one-hot encoding $\boldsymbol\tau'_{\mathit{tod}}$ by a trainable matrix $\mathbf{W}_{\mathit{tod}} \in \mathbb{R}^{96 \times 8}$ to achieve the time of day representation
  $\boldsymbol\tau_{\mathit{tod}} = \boldsymbol\tau'_{\mathit{tod}}\mathbf{W}_{\mathit{tod}}$ with dimensionality $8$.

\subsection{Day of Week Representation}
We represent the day of week in a manner similar to the time of day, but with $7$ dimensions in the one-hot encoding $\boldsymbol\tau'_{\mathit{dow}}$---one for each day of the week---and multiply $\boldsymbol\tau'_{\mathit{dow}}$ by a trainable weight matrix $\mathbf{W}_{\mathit{dow}} \in \mathbb{R}^{7 \times 8}$ to get an $8$-dimensional vector representation $\boldsymbol\tau_{\mathit{dow}}$ of the day of the week.


==> sections/experiments.tex <==
\section{Experiments}
We now proceed to evaluate our proposed method by comparing it against a number of baselines on the task of trip travel time estimation in the Danish road network.

\subsection{Data Set}
We extract the most important roads in the Danish road network from \gls{osm}~\citep{osm} and convert them into a graph representation as described in \cref{sec:roadNetworkModelling}.
This yields a graph with ?? nodes and ?? edges.
Then, we mapmatch a set of ?? vehicle trajectories to the road network and divide them into training, validation, and test sets.

\subsection{Algorithms}
\todo{Our method with and without observation updates}
\todo{Sum of independent estimations similar to relational fusion network paper}

\subsection{Experimental Setup}
We measure the average likelihood of the duration of each trip for our proposed method and all probabilistic baselines.
This allows us to evaluate how well our proposed method estimates the trip duration density function compared to the baselines.
\todo{Maybe it would be useful to have some idea of optimality? Maybe Oracle models?}

Not all the baselines are capable of estimating the trip duration density function. We therefore evaluate all models using \gls{mae}.
\todo{Write definition for MAE}
In the case of the non-probabilistic models, we measure the \gls{mae} between the model prediction and the ground truth trip duration.
For the probabilistic models, we measure the \gls{mae} between the most likely trip durations against the ground truth trip duration.

\subsection{Travel Time Estimation}

\subsection{Density Estimation}
\todo{Perhaps it is possible to estimate the density function of a given route s.t. one can see the probability distribution over trip durations by doing Monte Carlo simulation of each route.}

==> sections/method.tex <==
\section{Method}
Given an input route $R = (e_1, \dots, e_n)$ and a set of relevant historical trajectories $\mathcal{T}$ that traversed the route $\mathcal{T}$, we wish to output the travel time distribution $\Pr(T_R)$ of $R$.

\subsection{Route Convolutional Later}
Given a route $R (e_1, \dots, e_n)$ and feature matrices $X^V$, $X^E$, $X^B$, a route convolution performs transforms the route into a matrix $H_R = [h_1, \dots, h_n]$ where transformation of each edge $e_i \in R$ as follows
\begin{equation}\label{eq:route-convolution}
  h_i = \sigma(W \phi^E(e_{i-1}) \oplus \phi^B(b_{i-1}) \phi(e_i) \oplus \phi^B(b_{i+1}) \oplus \phi(e_{i+1}))
\end{equation}
where $b_{i-1} = (e_{i-1}, e_{i})$ and $b_{i+1} = (e_{i+1}, e_{i})$, $\oplus$ denotes vector concatenation, $\phi^E(e) = X^E_e$ encodes edges, and, for a between-edge $b=((u, v), (v, w))$, $\phi^B(b) = X^B_{b} \oplus X^V_{v}$ encodes between-edges and their connecting intersection. $\sigma$ is an activation function, $W$ a matrix of trainable weights, and $b$ is a bias term.
For each road segment $e_i \in R$, \cref{eq:route-convolution} captures the dependencies between the preceding and succeeding road segments.




































\begin{algorithm}
  \begin{algorithmic}
    \State{\Input{Route $R = (e_1, \dots, e_n)$, node feature matrix $X^V$, edge feature matrix $X^E$, between-edge feature matrix $X^B$, and the primal and dual graph representations of the road network $G^P$ and $G^D$, respectively.}}
    \State $(\theta^V, \theta^E, \theta^B) \gets \textsc{GCN}(X^V, X^E, X^B, G^P, G^D)$
    \State $\phi \gets ()$
    \For{$1 \leq i \leq n = (v_i, u_i) \in R$}
        \State \Let{$e_{i-1} = (v_{i-1}, u_{i-1})$} and \Let{$e_{i+1} = (v_{i+1}, u_{i+1})$} 
        \State Draw $\phi_{v_i}$ from $\Pr(\chi_{v_i} \mid \theta^V_{u_i})$
        \State Draw $\phi_{u_i}$ from $\Pr(\chi_{u_i} \mid \theta^V_{u_i})$
        \State Draw $\phi_{e_i}$ from $\Pr(\chi_{u_i} \mid \theta^V_{e_i})$
    \EndFor
  \end{algorithmic}
  \begin{algorithmic}
    \Function{DrawNodeRepresentations}{Graph Elements ()}
        \Comment{Draws a feature representation for input}
        return
    \EndFunction
  \end{algorithmic}
\end{algorithm}o

% Input
% 
% Route Convolution to encode the dependencies between edges in the route
\subsection{Stochastic Graph Convolutional Encoder}
% This may also contain observation update?
% Update before or after convolution?
\begin{itemize}
    \item Input: Node, edge, and between-edge feature matrices $X^V$, $X^E$, and $X^B$
    \item Output: Transformed node, edge, and between-edge feature matrices $Z^V$, $Z^E$, and $Z^B$ that are drawn from the probability distributions $\Pr(Z^V \mid \theta^V)$, $\Pr(Z^E \mid \theta^E)$, $\Pr(Z^B \mid \theta^B)$, respectively.
    \item Function: Stochastically transforms the node, edge, and between-edge features matrices by using a graph convolutional mechanism to enrich them with the characteristics of the local neighborhoods of nodes, edges, and between-edges, respectively. The encoder thus exploits spatial correlations among neighbors in the road network.
\end{itemize}

\subsection{Route Convolutional Layer}
\begin{itemize}
  \item Input: A route $R=(e_1, \dots, e_n)$ and the feature matrices $Z^V$, $Z^E$, and $Z^B$ from the Stochastic Graph Convolutional Encoder.
  \item Output: A sequence of stochastic variables $(T_1, \dots, T_n)$ that represent the segment-wise travel-time.
  \item Function: Estimates the travel time distribution for each road segment by taking into account its dependencies with the $k$ preceding and succeeding road segments in the route. Captures the spatial correlations within a route.
  \item Additional Info: Each stochastic variable $T_i$ is latent, but has observation variables $O_i$ associated with them, thus allowing the insertion of evidence from concrete traversals of the route. This enables the estimate to incorporate information from existing data.
\end{itemize}

\subsection{Aggregation}
\begin{itemize}
  \item Input: The sequence of stochastic variables $(T_1, \dots, T_n)$ outputted by the Route Convolutional Layer.
  \item Output: A travel time distribution $T_R$ for the route $R$.
  \item Function: 
\end{itemize}

\todo{You can use folded or truncated normal distributions to avoid modeling negative speeds}
\todo{Useful website on addition and multiplication with Gaussians: http://www.kaspercpa.com/statisticalreview.htm}
\begin{figure}
  \centering
  \input{illustrations/conceptual_framework.tikz.tex}
  \caption{Conceptual Framework\label{fig:conceptualFramework}}
  \todo{I believe the current to next arrow can be switched to produce an equivalent framework. This way we could reflect the dependencies using a HMM-like net.}
\end{figure}

We first construct a conceptual framework of our approach, illustrated in \cref{fig:conceptualFramework}.
We observe that the duration $D^T$ of a trip $T=(e_1, \dots, e_k)$ depends on the traversal speed $S_i$ across each segment $e_i$ in trip $T$.
Next, we observe that the traversal speed $S_i$ across segment $e_i \in R$ depends on the driving speed $S_{i-1}$ on the preceding segment $e_{i-1}$ in the trip.
For instance, if $e_{i-1}$ is highly congested (thus reducing the traversal speed), a vehicle takes longer to accelerate on segment $e_i$ than if $e_{i-1}$ had no congestion.
Similarly, the traversal speed $S_i$ across segment $e_i$ also depends on the traversal speed $S_{i+1}$ across the succeeding segment $e_{i+1}$: if the succeeding segment is congested, a vehicle slows down (voluntarily or otherwise).

Beside the traversal speed across preceding and succeeding segments, the trips $T_{1, i}$ and $T_{i, |P|}$, to and from segment $e_i$, respectively, also affects the traversal speed $S_i$ across $e_i$.
For instance, if a vehicle is required to make a sharp turn to transition from the preceding segment $e_{i-1}$ to a segment $e_i$, then the vehicle decelerates in anticipation of the turn which affects the speed $S_i$ on segment $e_i$ where time must be spent to accelerate again. Vice versa, if the vehicle is required to make a sharp turn onto the succeeding segment then the vehicle decelerates on segment $e_i$ in anticipation of the turn thus affecting the speed $S_i$ on the segment.
In general, the dependency on predecessor and successor segments is not limited to immediate successors. For instance, roundabouts consists of very short segments of a few meters where the immediate predecessors or successors in the trip fail to explain the driving speed completely.
\todo{May be relevant to cite some related work on aggregation models here.}


\subsection{SequentialRFN}
Sequential relational aggregation

\subsubsection{Prospect 1: Position-wise change}
Given a trip of nodes 
Compute a relational aggregate of each node in the trip as usual
Combine the aggregated representation with the sequential representation
 - E.g., by concatenating the representations and joining them through a neural network
Advantages: Could work for generic graph convolutional networks
Disadvantages:
 - How to take time into account sequentially?

\subsubsection{Prospect 2: Position-sensitive fusion function}
Given a trip of nodes
Compute a relational aggregate, but during fusion use the sequential representation to inform the aggregate
 - Could be quite expensive since a relational aggregate would be computed for each node in the trip
 - Is there a way to subvert this? Maybe use that additive fusion is essentially a sum?
    - Multiply the sequential representation by the number of neighbors and otherwise add the remaining transformations?
Advantages: Likely a more powerful model
Disadvantage:
 - Could be computationally expensive.
 - In addition, the relational fusion networks are relatively unknown and not yet an established method.
 - How to take time into account sequentially?


\subsubsection{Time-dependent model}

\paragraph{Estimation of Segment Arrival Times}
The arrival time at the $i$th segment of a trajectory $T=(e_1, \dots, e_2)$ is the arrival time at the previous segment plus the time it takes to traverse the previous segment.
Formally, the arrival time of the $i$th segment is
\begin{equation}\label{eq:arrival-time}
  T^{\tau}_i = T^{\tau}_{i-1} + \frac{l_{i-1}}{s_{i-1}}
\end{equation}
where $i > 1$ and $T^{\tau}_1$ is the starting time of the trip in number of time units (e.g., seconds) after midnight.
Here, $l_{i-1}$ is the length of segment $e_{i-1}$ and $s_{i-1}$ is the traversal speed across segment $e_{i-1}$.
In \cref{eq:arrival-time}, $s_i$ is an unknown quantity and we therefore estimate it using a neural network, but ensure that $s_i > 0$.
Note, however, that the estimate of $s_i$ is used only for estimating the arrival time, and not to estimate the travel time of trip $T$.

\paragraph{Arrival Time Encoding}
Travel times across a segment exhibit strong temporal correlations s.t.\ the travel time is similar within, e.g., a $15$~minute period.
We therefore desire an arrival time encoding that assign similar encoding to points in time that are temporally close.
To this end, we use a two-dimensional representation that encodes a point of time as a position on a ''clock'':
\begin{equation}\label{eq:time-encoding}
  f_{\tau}(\tau) = \begin{bmatrix}\cos(\tau) & \sin(\tau)\end{bmatrix}
\end{equation}
where $\tau$ is measured in time units after midnight.

The time encoding function $f_{\tau}$ has the property that, e.g., $0:05$ AM and $23:55$ are closer in, e.g., a Euclidean distance sense, than $0:05$ and $0:30$.
Thus, $f_{\tau}$ can capture the temporal correlations as desired.
However, in practice, there may also be correlations across different times of the day that are relatively distant such as morning and afternoon peaks.
In addition, we sum the time, edge, and positional encodings.
We therefore seek a time encoding that does not restrict the edge and positional encodings to any particular number of dimensions.
To this end, we transform the encoding as follows:
\begin{equation}
  \phi_{\tau}(\tau) = f_{\tau}(\tau)\mathbf{W}
\end{equation}
where $\mathbf{W} \in \mathbb{R}^{2 \times d}$ is a learnable projection matrix of parameters that projects the time encoding into a $d$-dimensional vector space.


Travel time across a route are temporally correlated s.t.\ 
Previous work has successfully leveraged the strong temporal correlations in driving speeds and travel times
A key property
A key feature of time


The intuition is that the arrival time at the $i$th segment 

Compute relational aggregate
When computing relational aggregate for each node v in a trip t:
    for each neighbor n of v:
        perform relational
Compute regular relational fusion aggregates 
For each entry 


\subsection{Loss Function}
\todo{Need to introduce that the travel time of a trip is a stochastic variable.}
We observe that, by the laws of physics, the travel time of a trip $T=(r_1, \dots, r_n)$ is equal to the sum of the travel time across each of its constituent edges $e_i \in T$.
Thus, the likelihood of a trip $T$ is the joint likelihood of the travel time across its constituent segments $\mathcal{L}(T) = \mathcal{L}(T_{0, 1}, T_{1, 2}, \dots, T_{n-1, n})$. We therefore aim to optimize this likelihood by minimizing the negative log-likelihood of the trips
\begin{equation}
  L_1(T) = \sum_{(e_i, s_i) \in T} -\ln\Bigg( L\bigg( \frac{l_i}{s_i} \bigg) \Bigg)
\end{equation}
where
\todo{Remove assumptions about the Gaussian nature of the speed variables.}
We compute a bipartite loss function
\begin{equation}
  \sum_{T \in \mathcal{T}} \alpha L_1(T) + (1-\alpha)L_2(T)
\end{equation}
where $\alpha, 0 \leq \alpha \leq 1$ regulates the importance between the two sub-losses $L_1$ and $L_2$.

The first sub-loss is used to encourage our method to learn accurate trip travel time estimates. It is defined as the negative log-likelihood of 
$L_1(T) = \sum_{}$


In other words, $y_T = \sum_{e_i \in T} y_{e_i}$ where $y_{e_i} = \frac{l_{e_i}}{s_{e_i}}$.
Motivated by this observation, we optimize our proposed method at the edge level.
Given a trip $T=(r_1, \dots, r_n)$, we minimize the \emph{negative log-likelihood} of the speed recorded for all road segments in the trip:
\begin{equation}\label{eq:edge-loss}
  L_2(T) = \sum_{(e_i, s_i) \in T, s_i \neq \varnothing} -\ln(\mathcal{L}(s_i))
\end{equation}
\todo{should probably normalize s.t.\ the number of known speeds does not affect the magnitude of the loss}

The loss in \cref{eq:edge-loss} encourages our method to be robust to the length of the trip since optimization is performed at the edge level.
However, as discussed previously, \gls{gps} sampling frequency can cause some road segments not to be associated with any speed and these road segments are filtered out during summation in \cref{eq:edge-loss}.
Road segments with missing recorded speeds tend to be relatively short segments and therefore the optimizing the loss in \cref{eq:edge-loss} encourages good predictions on longer segments which are unlikely to have missing speed records in trips.
To alleviate this problem we introduce another loss term to \cref{eq:edge-loss}:

We divide the loss function in two parts.
The first part optimizes the full trip duration prediction.
In order to train the network we 
We now present the loss function for our proposed methodWe design the loss functionw 
We compute a joint loss.
We predict both the 
By predicting  

A physical constraint in
A key property of our method is the reliance on the physical constraint that 


==> sections/preliminaries.tex <==
\section{Preliminaries}

\subsection{Modeling Road Networks}\label{sec:road-network-modelling}
\todo{Rewrite, currently taken directly from RFN paper}
We model a road network as an attributed directed graph $G = (V, E, A^V, A^E, A^B)$ where $V$ is the set of nodes and $E$ is the set of edges.
Each node $v \in V$ represents an intersection, and each edge $(u, v) \in E$ represents a road segment that enables traversal from $u$ to $v$.
Next, $A^V$ and $A^E$ maps intersections and road segments, respectively, to their attributes. In addition, $A^B$ maps a pair of road segments $(u, v), (v, w) \in E$ to their between-segment attributes such as the angle between $(u, v)$ and $(v, w)$ based on their spatial representation.
An example of a graph representation of the three-way intersection to the right in figure \cref{fig:compelling-example} is shown in \cref{fig:graph-rep-primal}.

Two intersections $u$ and $v$ in $V$ are adjacent if there exists a road segment $(u, v) \in E$ or $(v, u) \in E $. 
Similarly, two road segments $(u_1, v_1)$ and $(u_2, v_2)$ in $E$ are adjacent if $v_1 = u_2$ or $v_2 = u_1$. 
The function $N\colon V \cup E \xrightarrow{} 2^V \cup 2^E$ returns the neighborhood, i.e., the set of all adjacent intersections or road segments, of a road network element $g \in V \cup E$.
The dual graph representation of $G$ is then $G^D=(E, B)$ where $B = \big\{ \big((u, v), (v, w) \big) \mid (u, v), (v, w) \in E \big\}$ is the set of \emph{between-edges}.
Thus, $E$ and $B$ serve as the node and edge sets of the dual graph, respectively.
For disambiguation, we refer to $G$ as the primal graph representation.

\subsection{Routes and Trips}
A route $R = (e_1, \dots, e_n)$ is in a road network with primal graph $G^P=(V, E)$ and dual graph $G^P=(E, B)$ if $\forall e \in R, e \in E$ and $(e_i, e_{i+1}) \in B$ for $1 \leq i \leq n-1$. In addition, let $X^V$, $X^E$, and $X^B$ be the feature matrices that describe nodes, edges, and between-edges, respectively.

A \emph{trip} $T=(R, \tau)$ consists of a route $R = (e_1, \dots, e_n)$ in $G$ and a start time $\tau$.
For convenience, we say that a segment $e$ is in a trip $T=(R, \tau)$ if $e \in R$ and denote it using the notation $e \in T$.

\subsection{Feature Matrices}
The feature matrices $\mathbf{X}^V$, $\mathbf{X}^E$, and $\mathbf{X}^B$ encode the attributes of nodes ($A^V$), edges ($A^E$), and between-edges ($A^B$), respectively, as feature vectors s.t.\ each row row corresponds to a node, edge, or between-edge.
We use the notation $\mathbf{X}^V_v$, $\mathbf{X}^E_e$, and $\mathbf{X}^B_b$ to access the feature vectors of node $v$, edge $e$, and between-edge $b$, respectively.
In some contexts, we use the abbreviated notations $\mathbf{X}^V_i = \mathbf{X}^V_{v_i}$, $\mathbf{X}^E_i = \mathbf{X}^E_{e_i}$, and $\mathbf{X}^B_i = \mathbf{X}^B_{b_i}$.

\subsection{Route Convolutions}
A route convolution is a function $C$ takes as input a route $R = (e_1, \dots, e_n)$ and maps each edge $e \in R$ to a vector representation $c(v)$, s.t.\
\begin{equation}
  C(R) = \big(c(e_1), \dots, c(e_n)\big)
\end{equation}
In this framework, different choices of the convolution function $c$ lead to different route convolutions.
For instance, previous work \todo{citation needed} include one-dimensional convolutional layers in their architecture.
A one-dimensional convolutional layer with kernel size $k=1$ uses
\begin{equation}
  c(e_i) = \sigma\big(\mathbf{W} (\mathbf{X}^E_{i-1} \oplus \mathbf{X}^E_{i} \oplus \mathbf{X}^E_{i+1}) + \mathbf{b}\big),
\end{equation}
where $\sigma$ is an activation function, $\mathbf{W}$ is a learnable weight matrix, $\oplus$ denotes vector concatenation, and $\mathbf{b}$ is a bias term.
The term route convolution implies that information about the current edge $e_i$ is combined with that of its predecessors and successors in the route \todo{perhaps this is arguable}.
However, that is not necessarily the case.
For instance, if $c(e_i) = \sigma( \mathbf{W}\phi^E(e_i) + \mathbf{b})$.

\COMMENT{
\subsection{Modeling Trips}
A \emph{trip} in a road network $G=(V, E)$ is a pair $T=(R, \tau)$ that consists of a route $R = (e_1, \dots, e_n)$ in $G$ and a timestamp $\tau$ denoting the start of the trip.
For convenience, we say that a segment $e$ is in a trip $T=(R, \tau)$ if $e \in R$ and denote it using the notation $e \in T$.

The travel time of a trip $T$ is a random variable $\mathit{TT}_T$ that has the probability density function $\Pr(TT_T) = \prod_{e \in T} \Pr(TT_e)$ where $TT_e$ is random variable representing the travel time across segment $e$ in trip $T$.

A historical trip $T$
For the purposes of estimating 

A \emph{trip} is a sequence of \emph{trip records} $T=(r_1, \dots, r_n)$.
Each trip record $r_i$ in a trip $T$ is triple of the form $(e_i, \tau^a_i, \tau^d_i)$ where $e_i \in E$ is a road segment in a road network $G=(V, E)$. 
$\tau^a_i$ and $\tau^d_i$ are timestamps indicating the time and date the vehicle arrived to and departed from road segment $e_i$, respectively.
If the arrival and departure times are unknown, e.g., due to \gls{gps} sampling frequency, then $\tau^a_i = \varnothing$ and $\tau^d_i = \varnothing$.

The \emph{travel time} of a trip $T=(r_1, \dots, r_n)$ is the difference between the arrival time at the first road segment in the trip and the departure time from the last road segment in the trip, i.e., $y_T = \tau^d_n  - \tau^a_1$ where $\tau^d_n \neq \varnothing$ and $\tau^a_1 != \varnothing$.

\subsection{Relational Fusion Networks}
}


==> sections/related_work.tex <==
\section{Related Work}
% When Will You Arrive? Estimating Travel Time Based on Deep Neural Networks
%% Check their experiment baselines for some other related work


==> tmp.tex <==


\subsubsection{Bayesian Parameter Estimation of a Gaussian Mixture}
It is well-established in the literature that driving speeds do not follow any simple distribution, such as a Gaussian.
We therefore extend the single-component approach described in \cref{sec:parameter-estimation-gaussian} to the Gaussian mixture case.
In this case, the model $f$ is required to output prior parameters $w_0$, $\mu_0$, $\lambda_0$, $\alpha_0$, and $\beta_0$ for each of the $K$ components.

In brief, we introduce an update rule for the component weight of a Gaussian component $C_k$ in the mixture.
In addition, we modify the update rules in \cref{eq:parameter-update} s.t.\ the effect of a driving speed sample $d$ on the update of the prior parameters of a component $C_k$ is proportional to the probability $\Pr(C_k \mid d)$ that $d$ is generated by that component.
This ensures that the component means and variances do not all converge towards the sample mean and sample variance when there are is more than one component.

Given evidence $E = \{d_1, \dots, d_n\}$, we compute the posterior parameters of each Gaussian component $C_k$ in the mixture as follows.
\begin{equation}\label{eq:mixture-component-update}
\begin{split}
  w_n &= \frac{\kappa_0 w_0 + nw_d}
                   {\kappa_0 + n} \\
  \mu_n    &= \frac{\kappa_0 \mu_0 + p\bar{d}}
                   {\kappa_0 + p} \\
  \kappa_n &= \kappa_0 + p \\
  \alpha_n &= \alpha_0 + \frac{p}{2} \\
  \beta_n &= \beta_0 +
             \frac{1}{2} p S^2 +
             \frac{1}{2}\frac{\kappa_0 p {(\bar{d} - \mu_0)}^2}
                             {\kappa_0 + p}
\end{split}
\end{equation}
where
\begin{equation*}
  \begin{split}
    w_d &= \frac{1}{n} \sum_{i=1}^n\frac{\Pr(C_k \mid d_i)}{\sum_{j=1}^K\Pr(C_j \mid d_i)} \\
    p &= \sum_{i=1}^n \frac{{\Pr(C_k \mid d_i)}}
                {\sum_{j=1}^K \Pr(C_j \mid d_i)}, \\
    \bar{d} &= \frac{\sum_{i=1}^n \Pr(C_k \mid d_i) x_i}{\sum_{j=1}^n \Pr(C_k \mid d_j)}, \text{and} \\
    S^2 &= \frac{\sum_{i=1}^n{\Pr(C_k \mid d_i)(d_i - \bar{d})}^2}{\sum_{j=1}^n \Pr(C_k \mid d_j)}.
  \end{split}
\end{equation*}
Here, $w_d$ represents the component weight of component $C_k$ when estimated from the evidence $E$, and $p$ is a pseudo count representing the expected number of driving to have originated from component $C_k$. Similarly, $\bar{d}_k$ and $S^2_k$ is the expected sample mean and expected biased sample variance of the samples originating from component $C_k$.

The primary differences between the Gaussian parameter update rules in \cref{eq:parameter-update} and the Gaussian mixture update rules in \cref{eq:mixture-component-update} is that
\begin{enumerate}
  \item an update rule for the component weights in the mixture is introduced, and
  \item that the influence of the given samples in the update of a component $C_k$ is proportional to the number of expected samples originating from $C_k$.
\end{enumerate}
In other words, the samples given as evidence do not increase certainty about the mean $\mu$ and the variance $\sigma^2$ of component $C_k$ substantially if the samples are unlikely to have originated from component $C_k$.

